Search for the double-charmonium state with $\eta_c J/\psi$ at Belle

We measure the cross section of $e^+e^-\rightarrow\eta_c J/\psi$ at the $\Upsilon(nS) (n=1$ -- $5)$ on-resonance and 10.52 GeV off-resonance energy points using the full data sample collected by the Belle detector with an integrated luminosity of $955~\rm fb^{-1}$. We also search for double charmonium production in $e^+e^-\rightarrow\eta_c J/\psi$ via initial state radiation near the $\eta_c J/\psi$ threshold. No evident signal of the double charmonium state is found, but evidence for the $e^+e^-\rightarrow\eta_c J/\psi$ process is found with a statistical significance greater than $3.3\sigma$ near the $\eta_c J/\psi$ threshold. The average cross section near the threshold is measured and upper limits of cross sections are set for other regions.

==> authors-arXiv <==
Belle Collaboration: J. H. Yin, Y. B. Li, E. Won, I. Adachi, H. Aihara, S. Al Said, D. M. Asner, T. Aushev, R. Ayad, V. Babu, Sw. Banerjee, P. Behera, K. Belous, J. Bennett, M. Bessner, T. Bilka, D. Biswas, D. Bodrov, G. Bonvicini, J. Borah, A. Bozek, M. Bra\v{c}ko, P. Branchini, T. E. Browder, A. Budano, D. \v{C}ervenkov, M.-C. Chang, B. G. Cheon, K. Chilikin, H. E. Cho, K. Cho, S.-K. Choi, Y. Choi, S. Choudhury, D. Cinabro, J. Cochran, S. Das, G. De Nardo, G. De Pietro, R. Dhamija, F. Di Capua, J. Dingfelder, Z. Dole\v{z}al, T. V. Dong, D. Epifanov, T. Ferber, D. Ferlewicz, B. G. Fulsom, V. Gaur, A. Giri, P. Goldenzweig, E. Graziani, T. Gu, Y. Guan, K. Gudkova, C. Hadjivasiliou, S. Halder, T. Hara, K. Hayasaka, H. Hayashii, D. Herrmann, W.-S. Hou, C.-L. Hsu, T. Iijima, N. Ipsita, A. Ishikawa, R. Itoh, M. Iwasaki, W. W. Jacobs, Q. P. Ji, S. Jia, Y. Jin, K. K. Joo, J. Kahn, A. B. Kaliyar, T. Kawasaki, C. Kiesling, C. H. Kim, D. Y. Kim, K.-H. Kim, Y.-K. Kim, H. Kindo, K. Kinoshita, P. Kody\v{s}, A. Korobov, S. Korpar, E. Kovalenko, P. Kri\v{z}an, P. Krokovny, T. Kuhr, M. Kumar, R. Kumar, K. Kumara, T. Lam, J. S. Lange, S. C. Lee, L. K. Li, Y. Li, J. Libby, K. Lieret, Y.-R. Lin, D. Liventsev, M. Masuda, T. Matsuda, D. Matvienko, S. K. Maurya, F. Meier, M. Merola, F. Metzner, R. Mizuk, G. B. Mohanty, R. Mussa, I. Nakamura, D. Narwal, Z. Natkaniec, A. Natochii, L. Nayak, M. Nayak, N. K. Nisar, S. Nishida, S. Ogawa, H. Ono, P. Oskin, G. Pakhlova, S. Pardi, H. Park, J. Park, S.-H. Park, A. Passeri, S. Patra, S. Paul, R. Pestotnik, L. E. Piilonen, T. Podobnik, E. Prencipe, M. T. Prim, N. Rout, G. Russo, S. Sandilya, A. Sangal, L. Santelj, V. Savinov, G. Schnell, C. Schwanda, Y. Seino, K. Senyo, W. Shan, M. Shapkin, C. Sharma, J.-G. Shiu, E. Solovieva, M. Stari\v{c}, Z. S. Stottler, M. Sumihama, M. Takizawa, K. Tanida, F. Tenchini, R. Tiwary, M. Uchida, T. Uglov, Y. Unno, S. Uno, Y. Usov, S. E. Vahsen, G. Varner, A. Vinokurova, D. Wang, E. Wang, M.-Z. Wang, X. L. Wang, S. Watanuki, O. Werbycka, X. Xu, B. D. Yabsley, W. Yan, S. B. Yang, J. Yelton, Y. Yook, C. Z. Yuan, Z. P. Zhang, V. Zhilich, V. Zhukova

==> authors.tex <==
%%% Paper:    Double-charmonium state with eta_c J/psi
%%% Journal:  JHEP
%%% Contacts: J.H. Yin, Y.B. Li, E. Won
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{pub646} to insert this material into your latex file.
%%% Special instructions for JHEP:
%%%  1) add ",\hbox{$\dagger$}" inside the affiliation [...] and
%%%         "\note[$\dagger$]{Corresponding author.} after the corresponding author's name.
%%%  2) add  \emailAdd{...}" for the corresponding author at the end of this file.
\newcounter{AffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instGoettingen{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instBeihang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBINP{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instCMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPrague{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instChiba{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChonnam{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCAU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instDESY{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instDuke{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instITAR{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instEPFL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instJuelich{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFuJen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFudan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGifu{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSOKENDAI{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instGyeongsang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHanyang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKEK{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJPARC{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instHiroshima{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHUNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIKERBASQUE{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRomaTreINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTorinoINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTriesteINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIISER{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instIITBhubaneswar{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITGuwahati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITHyderabad{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITMadras{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIndiana{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIHEPRussia{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHEPHYVienna{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIHEPChina{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instChennai{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instISU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJAEA{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instKanagawa{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKarlsruhe{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKAU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKitasato{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKISTI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKoreaUnivKU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instKSU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyungpook{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instLNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGiessen{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instLuther{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMNITJaipur{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLMU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instSMI{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMEPhI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoya{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoyaKMI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNaraWu{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNCU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHSE{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNTUTaiwan{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNUUTaiwan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKrakow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNiigata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNDU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNSU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instOkinawa{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instOsakaMetropolitan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRCNP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPNNL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instPanjab{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instPeking{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMPP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPanjabPAU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRIKENMSL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instRIKENBNL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instSeoul{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSPU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoochow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoongsil{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSEU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaJSI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSKKU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTelAviv{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instToho{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTohoku{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTitech{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTokyoMetropolitan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaUNIV{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instRomaTreUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIJCLab{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBilbao{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBonn{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCincinnati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFlorida{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHawaii{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUniLJ{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLouisville{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMalaya{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMelbourne{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMississippi{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUOM{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNovaGorica{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUPES{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPittsburgh{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUSTC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSydney{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTabuk{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUTokyo{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instEri{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instIPMU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUtkal{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instVPI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instWayneState{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYamagata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYonsei{\protect\theAffiliationCounter}
\collaboration{The Belle Collaboration}
\author[\instKoreaUnivKU]{J.~H.~Yin,} % Korea
 \author[\instFudan]{Y.~B.~Li,} % Fudan
\author[\instKoreaUnivKU]{E.~Won,} % Korea
  \author[\instKEK,\instSOKENDAI]{I.~Adachi,} % KEK
% \author[\instLjubljanaJSI]{K.~Adamczyk,} % Ljubljana
% \author[\instKoreaUnivKU]{J.~K.~Ahn,} % Korea
  \author[\instUTokyo]{H.~Aihara,} % Tokyo
  \author[\instTabuk,\instKAU]{S.~Al~Said,} % Tabuk
  \author[\instBNL]{D.~M.~Asner,} % BNL
% \author[\instCincinnati]{H.~Atmacan,} % Cincinnati
% \author[\instBINP,\instNSU]{V.~Aulchenko,} % BINP
  \author[\instHSE]{T.~Aushev,} % HSE
  \author[\instTabuk]{R.~Ayad,} % Tabuk
% \author[\instTata]{T.~Aziz,} % Tata
  \author[\instIJCLab]{V.~Babu,} % IJCLab
% \author[\instIITBhubaneswar]{S.~Bahinipati,} % IITB
% \author[\instSydney]{A.~M.~Bakich,} % Sydney
% \author[\instPeking]{Y.~Ban,} % Peking
  \author[\instLouisville]{Sw.~Banerjee,} % Louisville
% \author[\instMelbourne]{E.~Barberio,} % Melbourne
% \author[\instKEK]{M.~Barrett,} % KEK
% \author[\instKarlsruhe]{M.~Bauer,} % Karlsruhe
  \author[\instIITMadras]{P.~Behera,} % IITM
  \author[\instIHEPRussia]{K.~Belous,} % Protvino
  \author[\instMississippi]{J.~Bennett,} % Mississippi
% \author[\instBonn]{F.~Bernlochner,} % Bonn
  \author[\instHawaii]{M.~Bessner,} % Hawaii
% \author[\instMEPhI]{D.~Besson,} % MEPhI
% \author[\instIISER]{V.~Bhardwaj,} % IISERM
% \author[\instIITGuwahati]{B.~Bhuyan,} % IITG
  \author[\instPrague]{T.~Bilka,} % Charles
% \author[\instLMU]{S.~Bilokin,} % LMU
  \author[\instLouisville]{D.~Biswas,} % Louisville
% \author[\instKEK]{T.~Bloomfield,} % KEK
% \author[\instBINP,\instNSU]{A.~Bobrov,} % BINP
  \author[\instHSE]{D.~Bodrov,} % HSE
% \author[\instBINP,\instNSU]{A.~Bondar,} % BINP
  \author[\instWayneState]{G.~Bonvicini,} % WayneState
  \author[\instIITGuwahati]{J.~Borah,} % IITG
  \author[\instKrakow]{A.~Bozek,} % Krakow
  \author[\instLjubljanaUM,\instLjubljanaJSI]{M.~Bra\v{c}ko,} % Ljubljana
  \author[\instRomaTreINFN]{P.~Branchini,} % RomaTre
  \author[\instHawaii]{T.~E.~Browder,} % Hawaii
  \author[\instRomaTreINFN]{A.~Budano,} % RomaTre
% \author[\instNapoliINFN,\instNapoliUNIV]{M.~Campajola,} % Napoli
% \author[\instDESY]{L.~Cao,} % DESY
  \author[\instPrague]{D.~\v{C}ervenkov,} % Charles
  \author[\instFuJen]{M.-C.~Chang,} % FuJen
% \author[\instNTUTaiwan]{P.~Chang,} % Taiwan
% \author[\instMPP]{V.~Chekelian,} % MPI
% \author[\instNCU]{A.~Chen,} % NCU
% \author[\instISU]{C.~Chen,} % ISU
% \author[\instUSTC]{Y.~Chen,} % USTC
% \author[\instNTUTaiwan]{Y.-T.~Chen,} % Taiwan
  \author[\instHanyang]{B.~G.~Cheon,} % Hanyang
  \author[\instBINP]{K.~Chilikin,} % BINP
  \author[\instHanyang]{H.~E.~Cho,} % Hanyang
  \author[\instKISTI]{K.~Cho,} % KISTI
% \author[\instYonsei]{S.-J.~Cho,} % Yonsei
  \author[\instCAU]{S.-K.~Choi,} % CAU
  \author[\instSKKU]{Y.~Choi,} % Sungkyunkwan
  \author[\instISU]{S.~Choudhury,} % ISU
  \author[\instWayneState]{D.~Cinabro,} % WayneState
  \author[\instISU]{J.~Cochran,} % ISU
% \author[\instDESY]{S.~Cunliffe,} % DESY
% \author[\instIPMU]{T.~Czank,} % IPMU
  \author[\instMNITJaipur]{S.~Das,} % MNIT
% \author[\instIITMadras]{N.~Dash,} % IITM
% \author[\instIJCLab]{G.~de~Marino,} % IJCLab
  \author[\instNapoliINFN,\instNapoliUNIV]{G.~De~Nardo,} % Napoli
  \author[\instKarlsruhe]{G.~De~Pietro,} % Karlsruhe
  \author[\instIITHyderabad]{R.~Dhamija,} % IITH
  \author[\instNapoliINFN,\instNapoliUNIV]{F.~Di~Capua,} % Napoli
  \author[\instBonn]{J.~Dingfelder,} % Bonn
  \author[\instPrague]{Z.~Dole\v{z}al,} % Charles
  \author[\instITAR]{T.~V.~Dong,} % DuyTan
% \author[\instMelbourne]{D.~Dossett,} % Melbourne
% \author[\instHawaii]{S.~Dubey,} % Hawaii
% \author[\instKarlsruhe]{P.~Ecker,} % Karlsruhe
  \author[\instBINP,\instNSU]{D.~Epifanov,} % BINP
% \author[\instKarlsruhe]{M.~Feindt,} % Karlsruhe
  \author[\instKarlsruhe]{T.~Ferber,} % Karlsruhe
  \author[\instMelbourne]{D.~Ferlewicz,} % Melbourne
% \author[\instGoettingen]{A.~Frey,} % Goettingen
  \author[\instPNNL]{B.~G.~Fulsom,} % PNNL
% \author[\instCMU]{R.~Garg,} % CMU
  \author[\instUPES]{V.~Gaur,} % UPES
% \author[\instBINP,\instNSU]{N.~Gabyshev,} % BINP
% \author[\instBINP,\instNSU]{A.~Garmash,} % BINP
  \author[\instIITHyderabad]{A.~Giri,} % IITH
  \author[\instKarlsruhe]{P.~Goldenzweig,} % Karlsruhe
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{B.~Golob,} % Ljubljana
% \author[\instUSTC]{G.~Gong,} % USTC
  \author[\instRomaTreINFN]{E.~Graziani,} % RomaTre
% \author[\instTUM]{D.~Greenwald,} % TUM
  \author[\instPittsburgh]{T.~Gu,} % Pittsburgh
  \author[\instCincinnati]{Y.~Guan,} % Cincinnati
  \author[\instBINP,\instNSU]{K.~Gudkova,} % BINP
  \author[\instPNNL]{C.~Hadjivasiliou,} % PNNL
% \author[\instHEPHYVienna]{H.~Haigh,} % Vienna
  \author[\instTata]{S.~Halder,} % Tata
% \author[\instBeihang]{X.~Han,} % Beihang
% \author[\instKEK]{K.~Hara,} % KEK
  \author[\instKEK,\instSOKENDAI]{T.~Hara,} % KEK
% \author[\instHawaii]{O.~Hartbrich,} % Hawaii
  \author[\instNiigata]{K.~Hayasaka,} % Niigata
  \author[\instNaraWu]{H.~Hayashii,} % Nara
% \author[\instTata]{S.~Hazra,} % Tata
% \author[\instBonn]{M.~T.~Hedges,} % Bonn
  \author[\instWayneState]{D.~Herrmann,} % WayneState
% \author[\instDESY]{M.~Hern\'{a}ndez~Villanueva,} % DESY
% \author[\instIPMU]{T.~Higuchi,} % IPMU
% \author[\instNagoya]{H.~Hirata,} % Nagoya
  \author[\instNTUTaiwan]{W.-S.~Hou,} % Taiwan
  \author[\instSydney]{C.-L.~Hsu,} % Sydney
% \author[\instNTUTaiwan]{K.~Huang,} % Taiwan
  \author[\instNagoyaKMI,\instNagoya]{T.~Iijima,} % Nagoya
% \author[\instNagoya]{K.~Inami,} % Nagoya
% \author[\instHEPHYVienna]{G.~Inguglia,} % Vienna
  \author[\instIITHyderabad]{N.~Ipsita,} % IITH
  \author[\instKEK,\instSOKENDAI]{A.~Ishikawa,} % KEK
  \author[\instKEK,\instSOKENDAI]{R.~Itoh,} % KEK
  \author[\instOsakaMetropolitan]{M.~Iwasaki,} % OsakaCity
% \author[\instKEK]{Y.~Iwasaki,} % KEK
% \author[\instTokyoMetropolitan]{S.~Iwata,} % TMU
  \author[\instIndiana]{W.~W.~Jacobs,} % Indiana
% \author[\instGyeongsang]{E.-J.~Jang,} % Gyeongsang
% \author[\instKyungpook]{H.~B.~Jeon,} % Kyungpook
  \author[\instHNU]{Q.~P.~Ji,} % HNU
  \author[\instSEU]{S.~Jia,} % SEU
  \author[\instTriesteINFN]{Y.~Jin,} % Trieste
  \author[\instChonnam]{K.~K.~Joo,} % Chonnam
  \author[\instKarlsruhe]{J.~Kahn,} % Karlsruhe
% \author[\instTokyoMetropolitan]{H.~Kakuno,} % TMU
% \author[\instIITGuwahati]{D.~Kalita,} % IITG
  \author[\instHEPHYVienna]{A.~B.~Kaliyar,} % Vienna
% \author[\instIPMU]{K.~H.~Kang,} % IPMU
% \author[\instISU]{S.~Kang,} % ISU
% \author[\instKrakow]{P.~Kapusta,} % Krakow
% \author[\instDESY]{G.~Karyan,} % DESY
% \author[\instNagoya]{Y.~Kato,} % Nagoya
% \author[\instChiba]{H.~Kawai,} % Chiba
  \author[\instKitasato]{T.~Kawasaki,} % Kitasato
% \author[\instKEK]{H.~Kichimi,} % KEK
  \author[\instMPP]{C.~Kiesling,} % MPI
  \author[\instHanyang]{C.~H.~Kim,} % Hanyang
  \author[\instSoongsil]{D.~Y.~Kim,} % Soongsil
% \author[\instKyungpook]{H.~J.~Kim,} % Kyungpook
  \author[\instKISTI]{K.-H.~Kim,} % KISTI
% \author[\instKoreaUnivKU]{K.~T.~Kim,} % Korea
% \author[\instSeoul]{S.~K.~Kim,} % Seoul
% \author[\instKoreaUnivKU]{Y.~J.~Kim,} % Korea
  \author[\instYonsei]{Y.-K.~Kim,} % Yonsei
% \author[\instVPI]{T.~D.~Kimmel,} % VPI
  \author[\instVPI,\instKEK]{H.~Kindo,} % VPI
  \author[\instCincinnati]{K.~Kinoshita,} % Cincinnati
% \author[\instDESY]{C.~Kleinwort,} % DESY
  \author[\instPrague]{P.~Kody\v{s},} % Charles
% \author[\instDESY]{I.~Komarov,} % DESY
% \author[\instKitasato]{T.~Konno,} % Kitasato
  \author[\instBINP,\instNSU]{A.~Korobov,} % BINP
  \author[\instLjubljanaUM,\instLjubljanaJSI]{S.~Korpar,} % Ljubljana
  \author[\instBINP,\instNSU]{E.~Kovalenko,} % BINP
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{P.~Kri\v{z}an,} % Ljubljana
% \author[\instMississippi]{R.~Kroeger,} % Mississippi
% \author[\instMelbourne]{J.-F.~Krohn,} % Melbourne
  \author[\instBINP,\instNSU]{P.~Krokovny,} % BINP
  \author[\instLMU]{T.~Kuhr,} % LMU
  \author[\instIISER]{M.~Kumar,} % IISERM
  \author[\instPanjabPAU]{R.~Kumar,} % Punjab
  \author[\instMississippi]{K.~Kumara,} % Mississippi
% \author[\instTokyoMetropolitan]{T.~Kumita,} % TMU
% \author[\instChiba]{E.~Kurihara,} % Chiba
% \author[\instBINP,\instNSU]{A.~Kuzmin,} % BINP
% \author[\instPrague]{P.~Kvasni\v{c}ka,} % Charles
% \author[\instYonsei]{Y.-J.~Kwon,} % Yonsei
% \author[\instKEK]{Y.-T.~Lai,} % KEK
% \author[\instMNITJaipur]{K.~Lalwani,} % MNIT
  \author[\instVPI]{T.~Lam,} % VPI
  \author[\instGiessen]{J.~S.~Lange,} % Giessen
% \author[\instRomaTreINFN,\instRomaTreUNIV]{M.~Laurenza,} % RomaTre
% \author[\instHanyang]{I.~S.~Lee,} % Hanyang
% \author[\instSeoul]{J.~K.~Lee,} % Seoul
  \author[\instKyungpook]{S.~C.~Lee,} % Kyungpook
% \author[\instKEK]{D.~Levit,} % KEK
% \author[\instBonn]{P.~Lewis,} % Bonn
% \author[\instLNNU]{C.~H.~Li,} % LNNU
% \author[\instKyungpook]{J.~Li,} % Kyungpook
  \author[\instCincinnati]{L.~K.~Li,} % Cincinnati
% \author[\instFudan]{S.~X.~Li,} % Fudan
  \author[\instFudan]{Y.~Li,} % Fudan
% \author[\instMPP]{L.~Li~Gioi,} % MPI
  \author[\instIITMadras]{J.~Libby,} % IITM
  \author[\instLMU]{K.~Lieret,} % LMU
  \author[\instNTUTaiwan]{Y.-R.~Lin,} % Taiwan
% \author[\instHiroshima]{Z.~Liptak,} % Hiroshima
  \author[\instWayneState,\instKEK]{D.~Liventsev,} % WayneState
% \author[\instFudan]{T.~Luo,} % Fudan
% \author[\instRIKENMSL]{Y.~Ma,} % NPC
% \author[\instUOM]{J.~MacNaughton,} % NPC
% \author[\instDESY]{A.~Martini,} % DESY
  \author[\instEri,\instRCNP]{M.~Masuda,} % NPC
  \author[\instUOM]{T.~Matsuda,} % NPC
  \author[\instBINP,\instNSU]{D.~Matvienko,} % BINP
  \author[\instIITGuwahati]{S.~K.~Maurya,} % IITG
  \author[\instDuke]{F.~Meier,} % Duke
  \author[\instNapoliINFN,\instNapoliUNIV]{M.~Merola,} % Napoli
  \author[\instBonn]{F.~Metzner,} % Bonn
% \author[\instNaraWu,\instKEK]{K.~Miyabayashi,} % Nara
% \author[\instKEK,\instSOKENDAI]{H.~Miyake,} % KEK
% \author[\instNiigata]{H.~Miyata,} % Niigata
  \author[\instHSE]{R.~Mizuk,} % HSE
  \author[\instTata]{G.~B.~Mohanty,} % Tata
% \author[\instKoreaUnivKU]{H.~K.~Moon,} % Korea
% \author[\instSeoul]{T.~J.~Moon,} % Seoul
% \author[\instMPP]{H.-G.~Moser,} % MPI
% \author[\instHEPHYVienna]{M.~Mrvar,} % Vienna
% \author[\instKarlsruhe]{T.~M\"uller,} % Karlsruhe
  \author[\instTorinoINFN]{R.~Mussa,} % Torino
  \author[\instKEK,\instSOKENDAI]{I.~Nakamura,} % KEK
% \author[\instKEK]{K.~R.~Nakamura,} % KEK
% \author[\instOsakaMetropolitan]{E.~Nakano,} % OsakaCity
% \author[\instRCNP]{T.~Nakano,} % NPC
% \author[\instKEK,\instSOKENDAI]{M.~Nakao,} % KEK
% \author[\instKEK,\instSOKENDAI]{H.~Nakayama,} % KEK
% \author[\instNTUTaiwan]{H.~Nakazawa,} % Taiwan
  \author[\instIITGuwahati]{D.~Narwal,} % IITG
  \author[\instKrakow]{Z.~Natkaniec,} % Krakow
  \author[\instHawaii]{A.~Natochii,} % Hawaii
  \author[\instIITHyderabad]{L.~Nayak,} % IITH
  \author[\instTelAviv]{M.~Nayak,} % TelAviv
% \author[\instDESY]{C.~Niebuhr,} % DESY
% \author[\instKSU]{M.~Niiyama,} % NPC
  \author[\instBNL]{N.~K.~Nisar,} % BNL
  \author[\instKEK,\instSOKENDAI]{S.~Nishida,} % KEK
% \author[\instHawaii]{K.~Nishimura,} % Hawaii
% \author[\instNiigata]{K.~Ogawa,} % Niigata
  \author[\instToho]{S.~Ogawa,} % Toho
% \author[\instKanagawa]{S.~Okuno,} % Kanagawa
% \author[\instCAU]{S.~L.~Olsen,} % CAU
  \author[\instNDU,\instNiigata]{H.~Ono,} % NihonDental
% \author[\instUTokyo]{Y.~Onuki,} % Tokyo
  \author[\instIJCLab]{P.~Oskin,} % IJCLab
% \author[\instKEK,\instSOKENDAI]{H.~Ozaki,} % KEK
% \author[\instHSE]{P.~Pakhlov,} % HSE
  \author[\instHSE]{G.~Pakhlova,} % HSE
% \author[\instPittsburgh]{T.~Pang,} % Pittsburgh
  \author[\instNapoliINFN]{S.~Pardi,} % Napoli
  \author[\instKyungpook]{H.~Park,} % Kyungpook
  \author[\instYonsei]{J.~Park,} % Yonsei
  \author[\instKEK]{S.-H.~Park,} % KEK
  \author[\instRomaTreINFN]{A.~Passeri,} % RomaTre
  \author[\instLouisville]{S.~Patra,} % Louisville
  \author[\instTUM,\instMPP]{S.~Paul,} % TUM
% \author[\instLuther]{T.~K.~Pedlar,} % Luther
  \author[\instLjubljanaJSI]{R.~Pestotnik,} % Ljubljana
% \author[\instMelbourne]{F.~Pham,} % Melbourne
  \author[\instVPI]{L.~E.~Piilonen,} % VPI
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{T.~Podobnik,} % Ljubljana
% \author[\instHSE]{V.~Popov,} % HSE
% \author[\instISU]{S.~Prell,} % ISU
  \author[\instGiessen]{E.~Prencipe,} % Giessen
  \author[\instBonn]{M.~T.~Prim,} % Bonn
% \author[\instOkinawa]{M.~V.~Purohit,} % OIST
% \author[\instTUM]{A.~Rabusov,} % TUM
% \author[\instLMU]{M.~Ritter,} % LMU
% \author[\instDESY]{M.~R\"{o}hrken,} % DESY
% \author[\instDESY]{A.~Rostomyan,} % DESY
  \author[\instTriesteINFN]{N.~Rout,} % Trieste
% \author[\instKrakow]{M.~Rozanska,} % Krakow
  \author[\instNapoliUNIV]{G.~Russo,} % Napoli
% \author[\instISU]{D.~Sahoo,} % ISU
% \author[\instKEK,\instSOKENDAI]{Y.~Sakai,} % KEK
% \author[\instMalaya,\instLMU]{M.~Salehi,} % Malaya
  \author[\instIITHyderabad]{S.~Sandilya,} % IITH
  \author[\instCincinnati]{A.~Sangal,} % Cincinnati
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{L.~Santelj,} % Ljubljana
% \author[\instTohoku]{T.~Sanuki,} % Tohoku
  \author[\instPittsburgh]{V.~Savinov,} % Pittsburgh
% \author[\instLMU]{P.~Schmolz,} % LMU
% \author[\instEPFL]{O.~Schneider,} % Lausanne
  \author[\instBilbao,\instIKERBASQUE]{G.~Schnell,} % Bilbao
% \author[\instHawaii]{J.~Schueler,} % Hawaii
  \author[\instHEPHYVienna]{C.~Schwanda,} % Vienna
% \author[\instCincinnati]{A.~J.~Schwartz,} % Cincinnati
% \author[\instGoettingen]{B.~Schwenker,} % Goettingen
% \author[\instRIKENBNL]{R.~Seidl,} % RIKEN
  \author[\instNiigata]{Y.~Seino,} % Niigata
  \author[\instYamagata]{K.~Senyo,} % Yamagata
% \author[\instNagoya]{O.~Seon,} % Nagoya
% \author[\instMelbourne]{M.~E.~Sevior,} % Melbourne
  \author[\instHUNNU]{W.~Shan,} % HUNNU
  \author[\instIHEPRussia]{M.~Shapkin,} % Protvino
  \author[\instMNITJaipur]{C.~Sharma,} % MNIT
% \author[\instHawaii]{V.~Shebalin,} % Hawaii
% \author[\instFudan]{C.~P.~Shen,} % Fudan
% \author[\instToho]{H.~Shibuya,} % Toho
  \author[\instNTUTaiwan]{J.-G.~Shiu,} % Taiwan
% \author[\instBINP,\instNSU]{B.~Shwartz,} % BINP
% \author[\instHawaii]{A.~Sibidanov,} % Hawaii
% \author[\instMPP]{F.~Simon,} % MPI
% \author[\instPanjab,\instUPES]{J.~B.~Singh,} % Panjab
% \author[\instChennai]{R.~Sinha,} % IMSC
% \author[\instMelbourne]{K.~Smith,} % Melbourne
% \author[\instIHEPRussia]{A.~Sokolov,} % Protvino
% \author[\instDESY]{Y.~Soloviev,} % DESY
  \author[\instBINP]{E.~Solovieva,} % BINP
% \author[\instNovaGorica]{S.~Stani\v{c},} % NovaGorica
  \author[\instLjubljanaJSI]{M.~Stari\v{c},} % Ljubljana
  \author[\instVPI]{Z.~S.~Stottler,} % VPI
% \author[\instPNNL]{J.~F.~Strube,} % PNNL
% \author[\instKrakow]{J.~Stypula,} % Krakow
  \author[\instGifu,\instRCNP]{M.~Sumihama,} % NPC
% \author[\instKEK,\instSOKENDAI,\instNaraWu]{K.~Sumisawa,} % KEK
% \author[\instTokyoMetropolitan]{T.~Sumiyoshi,} % TMU
% \author[\instBonn]{W.~Sutcliffe,} % Bonn
% \author[\instKEK]{S.~Y.~Suzuki,} % KEK
  \author[\instSPU,\instJPARC,\instRIKENMSL]{M.~Takizawa,} % NPC
% \author[\instTorinoINFN]{U.~Tamponi,} % Torino
% \author[\instKEK,\instSOKENDAI]{S.~Tanaka,} % KEK
% \author[\instFudan]{S.~S.~Tang,} % Fudan
  \author[\instJAEA]{K.~Tanida,} % NPC
% \author[\instKEK]{N.~Taniguchi,} % KEK
% \author[\instFlorida]{Y.~Tao,} % Florida
% \author[\instMelbourne]{G.~N.~Taylor,} % Melbourne
  \author[\instPisaINFN,\instPisaUNIV]{F.~Tenchini,} % Pisa
% \author[\instOsakaMetropolitan]{Y.~Teramoto,} % OsakaCity
% \author[\instJuelich]{A.~Thampi,} % Juelich
  \author[\instTata]{R.~Tiwary,} % Tata
% \author[\instIJCLab]{K.~Trabelsi,} % IJCLab
% \author[\instKEK,\instSOKENDAI]{T.~Tsuboyama,} % KEK
% \author[\instNagoya]{N.~Tsuzuki,} % Nagoya
  \author[\instTitech]{M.~Uchida,} % NPC
% \author[\instKEK,\instSOKENDAI]{I.~Ueda,} % KEK
% \author[\instKEK,\instSOKENDAI]{S.~Uehara,} % KEK
  \author[\instHSE]{T.~Uglov,} % HSE
  \author[\instHanyang]{Y.~Unno,} % Hanyang
% \author[\instNiigata]{K.~Uno,} % Niigata
  \author[\instKEK,\instSOKENDAI]{S.~Uno,} % KEK
% \author[\instMelbourne]{P.~Urquijo,} % Melbourne
% \author[\instKEK,\instSOKENDAI]{Y.~Ushiroda,} % KEK
  \author[\instBINP,\instNSU]{Y.~Usov,} % BINP
  \author[\instHawaii]{S.~E.~Vahsen,} % Hawaii
  \author[\instHawaii]{G.~Varner,} % Hawaii
% \author[\instSydney]{K.~E.~Varvell,} % Sydney
  \author[\instBINP,\instNSU]{A.~Vinokurova,} % BINP
% \author[\instBINP]{V.~Vorobyev,} % BINP
% \author[\instDuke]{A.~Vossen,} % Duke
% \author[\instKEK]{E.~Waheed,} % KEK
% \author[\instMPP]{B.~Wang,} % MPI
% \author[\instNUUTaiwan]{C.~H.~Wang,} % NUU
  \author[\instFlorida]{D.~Wang,} % Florida
  \author[\instPittsburgh]{E.~Wang,} % Pittsburgh
  \author[\instNTUTaiwan]{M.-Z.~Wang,} % Taiwan
  \author[\instFudan]{X.~L.~Wang,} % Fudan
% \author[\instNiigata]{M.~Watanabe,} % Niigata
% \author[\instKanagawa]{Y.~Watanabe,} % Kanagawa
  \author[\instYonsei]{S.~Watanuki,} % Yonsei
% \author[\instDESY]{S.~Wehle,} % DESY
  \author[\instTriesteINFN]{O.~Werbycka,} % Trieste
% \author[\instSMI]{E.~Widmann,} % Vienna
% \author[\instKrakow]{J.~Wiechczynski,} % Krakow
  \author[\instSoochow]{X.~Xu,} % Soochow
  \author[\instSydney]{B.~D.~Yabsley,} % Sydney
% \author[\instKEK]{S.~Yamada,} % KEK
% \author[\instTohoku]{H.~Yamamoto,} % Tohoku
  \author[\instUSTC]{W.~Yan,} % USTC
  \author[\instKoreaUnivKU]{S.~B.~Yang,} % Korea
% \author[\instDESY]{H.~Ye,} % DESY
  \author[\instFlorida]{J.~Yelton,} % Florida
  \author[\instIHEPChina]{Y.~Yook,} % IHEP
  \author[\instIHEPChina]{C.~Z.~Yuan,} % IHEP
% \author[\instBeihang]{L.~Yuan,} % Beihang
% \author[\instNiigata]{Y.~Yusa,} % Niigata
% \author[\instISU]{Y.~Zhai,} % ISU
% \author[\instIHEPChina]{J.~Zhang,} % IHEP
  \author[\instUSTC]{Z.~P.~Zhang,} % USTC
  \author[\instBINP,\instNSU]{V.~Zhilich,} % BINP
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{V.~Zhukova,} % Ljubljana
% \author[\instBINP,\instNSU]{V.~Zhulanov} % BINP
%%%\affiliation[\instGoettingen]{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
%%%\affiliation[\instBeihang]{Beihang University, Beijing 100191, China}
\affiliation[\instBNL]{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\affiliation[\instBINP]{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
%%%\affiliation[\instCMU]{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\affiliation[\instPrague]{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
%%%\affiliation[\instChiba]{Chiba University, Chiba 263-8522, Japan}
\affiliation[\instChonnam]{Chonnam National University, Gwangju 61186, South Korea}
\affiliation[\instCAU]{Chung-Ang University, Seoul 06974, South Korea}
%%%\affiliation[\instDESY]{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\affiliation[\instDuke]{Duke University, Durham, North Carolina 27708, U.S.A.}
\affiliation[\instITAR]{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
%%%\affiliation[\instEPFL]{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015, Switzerland}
%%%\affiliation[\instJuelich]{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich, Germany}
\affiliation[\instFuJen]{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\affiliation[\instFudan]{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\affiliation[\instGifu]{Gifu University, Gifu 501-1193, Japan}
\affiliation[\instSOKENDAI]{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
%%%\affiliation[\instGyeongsang]{Gyeongsang National University, Jinju 52828, South Korea}
\affiliation[\instHanyang]{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
\affiliation[\instHNU]{Henan Normal University, Xinxiang 453007, China}
\affiliation[\instKEK]{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\affiliation[\instJPARC]{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
%%%\affiliation[\instHiroshima]{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\affiliation[\instHUNNU]{Hunan Normal University, Changsha 410081, China}
\affiliation[\instIKERBASQUE]{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao, Spain}
\affiliation[\instNapoliINFN]{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\affiliation[\instPisaINFN]{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\affiliation[\instRomaTreINFN]{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instTorinoINFN]{INFN Sezione di Torino, I-10125 Torino, Italy}
\affiliation[\instTriesteINFN]{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\affiliation[\instIISER]{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
%%%\affiliation[\instIITBhubaneswar]{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\affiliation[\instIITGuwahati]{Indian Institute of Technology Guwahati, Assam 781039, India}
\affiliation[\instIITHyderabad]{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\affiliation[\instIITMadras]{Indian Institute of Technology Madras, Chennai 600036, India}
\affiliation[\instIndiana]{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\affiliation[\instIHEPRussia]{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\affiliation[\instHEPHYVienna]{Institute of High Energy Physics, Vienna 1050, Austria}
\affiliation[\instIHEPChina]{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
%%%\affiliation[\instChennai]{Institute of Mathematical Sciences, Chennai 600113, India}
\affiliation[\instISU]{Iowa State University, Ames, Iowa 50011, U.S.A.}
\affiliation[\instJAEA]{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
%%%\affiliation[\instKanagawa]{Kanagawa University, Yokohama 221-8686, Japan}
\affiliation[\instKarlsruhe]{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\affiliation[\instKAU]{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589, Saudi Arabia}
\affiliation[\instKitasato]{Kitasato University, Sagamihara 252-0373, Japan}
\affiliation[\instKISTI]{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\affiliation[\instKoreaUnivKU]{Korea University, Seoul 02841, South Korea}
%%%\affiliation[\instKSU]{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\affiliation[\instKyungpook]{Kyungpook National University, Daegu 41566, South Korea}
%%%\affiliation[\instLNNU]{Liaoning Normal University, Dalian 116029, China}
\affiliation[\instGiessen]{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
%%%\affiliation[\instLuther]{Luther College, Decorah, Iowa 52101, U.S.A.}
\affiliation[\instMNITJaipur]{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\affiliation[\instLMU]{Ludwig Maximilians University, 80539 Munich, Germany}
%%%\affiliation[\instSMI]{Stefan Meyer Institute for Subatomic Physics, Vienna 1090, Austria}
%%%\affiliation[\instMEPhI]{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\affiliation[\instNagoya]{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\affiliation[\instNagoyaKMI]{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
\affiliation[\instNaraWu]{Nara Women's University, Nara 630-8506, Japan}
%%%\affiliation[\instNCU]{National Central University, Chung-li 32054, Taiwan}
\affiliation[\instHSE]{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\affiliation[\instNTUTaiwan]{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
%%%\affiliation[\instNUUTaiwan]{National United University, Miao Li 36003, Taiwan}
\affiliation[\instKrakow]{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\affiliation[\instNiigata]{Niigata University, Niigata 950-2181, Japan}
\affiliation[\instNDU]{Nippon Dental University, Niigata 951-8580, Japan}
\affiliation[\instNSU]{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
%%%\affiliation[\instOkinawa]{Okinawa Institute of Science and Technology, Okinawa 904-0495, Japan}
\affiliation[\instOsakaMetropolitan]{Osaka Metropolitan University, Osaka 558-8585, Japan}
\affiliation[\instRCNP]{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\affiliation[\instPNNL]{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
%%%\affiliation[\instPanjab]{Panjab University, Chandigarh 160014, India}
%%%\affiliation[\instPeking]{Peking University, Beijing 100871, China}
\affiliation[\instMPP]{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\affiliation[\instPanjabPAU]{Punjab Agricultural University, Ludhiana 141004, India}
\affiliation[\instRIKENMSL]{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
%%%\affiliation[\instRIKENBNL]{RIKEN BNL Research Center, Upton, New York 11973, U.S.A.}
%%%\affiliation[\instSeoul]{Seoul National University, Seoul 08826, South Korea}
\affiliation[\instSPU]{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\affiliation[\instSoochow]{Soochow University, Suzhou 215006, China}
\affiliation[\instSoongsil]{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\affiliation[\instSEU]Southeast University, Nanjing 211189, China}
\affiliation[\instLjubljanaJSI]{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\affiliation[\instSKKU]{Sungkyunkwan University, Suwon 16419, South Korea}
\affiliation[\instTata]{Tata Institute of Fundamental Research, Mumbai 400005, India}
\affiliation[\instTUM]{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\affiliation[\instTelAviv]{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\affiliation[\instToho]{Toho University, Funabashi 274-8510, Japan}
%%%\affiliation[\instTohoku]{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\affiliation[\instTitech]{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
%%%\affiliation[\instTokyoMetropolitan]{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\affiliation[\instNapoliUNIV]{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\affiliation[\instPisaUNIV]{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
%%%\affiliation[\instRomaTreUNIV]{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instIJCLab]{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affiliation[\instBilbao]{Department of Physics \& EHU Quantum Center, University of the Basque Country UPV/EHU, 48080 Bilbao, Spain}
\affiliation[\instBonn]{University of Bonn, 53115 Bonn, Germany}
\affiliation[\instCincinnati]{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\affiliation[\instFlorida]{University of Florida, Gainesville, Florida 32611, U.S.A.}
\affiliation[\instHawaii]{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\affiliation[\instLjubljanaUniLJ]{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\affiliation[\instLouisville]{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
%%%\affiliation[\instMalaya]{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
\affiliation[\instLjubljanaUM]{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\affiliation[\instMelbourne]{School of Physics, University of Melbourne, Victoria 3010, Australia}
\affiliation[\instMississippi]{University of Mississippi, University, Mississippi 38677, U.S.A.}
\affiliation[\instUOM]{University of Miyazaki, Miyazaki 889-2192, Japan}
%%%\affiliation[\instNovaGorica]{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\affiliation[\instUPES]{University of Petroleum and Energy Studies, Dehradun 248007, India}
\affiliation[\instPittsburgh]{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\affiliation[\instUSTC]{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\affiliation[\instSydney]{School of Physics, University of Sydney, New South Wales 2006, Australia}
\affiliation[\instTabuk]{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\affiliation[\instUTokyo]{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\affiliation[\instEri]{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
%%%\affiliation[\instIPMU]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
%%%\affiliation[\instUtkal]{Utkal University, Bhubaneswar 751004, India}
\affiliation[\instVPI]{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\affiliation[\instWayneState]{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\affiliation[\instYamagata]{Yamagata University, Yamagata 990-8560, Japan}
\affiliation[\instYonsei]{Yonsei University, Seoul 03722, South Korea}
